New constraints on the structure and dynamics of black hole jets

Accreting black holes produce powerful relativistic plasma jets which emit radiation across all observable wavelengths but the details of the initial acceleration and confinement of the jet are uncertain. We apply an innovative new model that allows us to determine key properties of the acceleration zone via multi-frequency observations. The central component of the model is a relativistic steady-state fluid flow, and the emission from physically distinct regions can be seen to contribute to different energy bands in the overall spectrum. By fitting with unprecedented accuracy to 42 simultaneous multiwavelength blazar spectra we are able to constrain the location of the brightest synchrotron emitting region, and show that there must be a linear relation between the jet power and the radius of the brightest region of the jet. We also find a correlation between the length of the accelerating region and the maximum bulk Lorentz factor of the jet and find evidence for a bimodal distribution of accretion rates in the blazar population. This allows us to put constraints on the basic dynamical and structural properties of blazar jets and to understand the underlying physical differences which result in the blazar sequence.

==> Chapter5.tex <==
\chapter{Understanding the physics behind the blazar population}
\ifpdf
    \graphicspath{{Chapter5/Chapter5Figs/PNG/}{Chapter5/Chapter5Figs/PDF/}{Chapter5/Chapter5Figs/}}
\else
    \graphicspath{{Chapter5/Chapter5Figs/EPS/}{Chapter5/Chapter5Figs/}}
\fi

This is the concluding Chapter of my work modelling blazars. In this Chapter I use the model developed in Chapters 2-5 to fit to the remaining 32 blazars with simultaneous multiwavelength spectra and redshifts available from the {\it Fermi} sample (\cite{2010ApJ...716...30A}). The model fits with unprecedented detail to all these blazars. I find strong empirical evidence for the predicted physical relation in Chapters 4 and 5; namely that the radius of the transition region and maximum bulk Lorentz factor increase with jet power. This is important since it provides an explanation for the basis of the blazar sequence.

I conclude that if black hole mass measurements can be believed, my results offer strong evidence for a scenario in which two accretion modes exist in blazars resulting in BL Lac and FSRQ type jets, analogous to the relationship between accretion mode and jet properties in X-ray binary systems. These sub-Eddington and Eddington accretion modes result in BL Lacs and FSRQs which have the expected properties of FRI and FRII jets observed close to the line of sight, as suggested by unification. These results are very exciting as they offer explanations and evidence for many long standing questions and hypotheses about blazars and AGN jets.

\section{Introduction}

%A fraction of supermassive black holes are observed to produce powerful, relativistic plasma jets. Blazars are the most extreme class of these jets in which we observe directly down the jet axis so the emission is strongly Doppler-boosted. These jets are created by the accretion of a magnetised plasma onto a spinning supermassive black hole at the centre of a galaxy. Jets are thought to be composed from electron positron pairs and are accelerated to within a fraction of the speed of light by the magnetic pressure gradient of a rotating, expanding helical magnetic field tied to the event horizon of a spinning black hole. 

%Jets are observed to emit radiation across the entire electromagnetic spectrum, however, existing compact emission models have been unable to constrain the structure and dynamics of these jets. Here we show an approximately linear relation exists between the jet power and the radius of the jet where the jet stops accelerating and first comes into equipartition. This is the first time that multifrequency observations including radio data have been successfully modelled for a large sample of blazars and we use these results to understand the physical reason behind the blazar sequence, which has long been a puzzle. We find evidence for a distinct difference in the properties of BL Lacs and FSRQs corresponding to FRI and FRII jets respectively and relate this to the bimodal accretion rate of BL Lacs and FSRQs if we assume both have similar black hole mass distributions.  

It has recently been observed that the jet in M87 has a parabolic base out to $10^{5}$ Schwarzschild radii becoming conical beyond this distance (\cite{2011arXiv1110.1793A}). This is consistent with state of the art numerical simulations which show the jet base starts magnetically dominated and accelerates in the parabolic region reaching a terminal bulk Lorentz factor at equipartition after which the jet becomes ballistic and conical (\cite{2006MNRAS.368.1561M}, \cite{2009MNRAS.394.1182K}, \cite{2010ApJ...711...50T} and \cite{2012MNRAS.423.3083M}). In this Chapter we use a model for the emission of a realistic jet motivated by and consistent with these recent observations and simulations in order to test this emerging picture of jets and to try to determine their properties.

We use the realistic extended jet model for emission from Chapters 2-5 (based on \cite{2012MNRAS.423..756P}, \cite{2013MNRAS.429.1189P}, \cite{2013MNRAS.431.1840P} and \cite{2013MNRASP4.}) to fit to the remaining 32 blazars with simultaneous multiwavelength observations and redshifts from the {\it Fermi} sample (\cite{2010ApJ...716...30A}). This model is the first to be able to simultaneously match the observations of blazars across all frequencies, including radio data, by considering the extended large scale structure of the jet. In being able to match the radio observations of jets we are able to tightly constrain the radius of the jet at the transition region by fitting the break frequency above which the synchrotron emission becomes optically thin (which sensitively depends on the radius at which the jet first approaches equipartition). This is the first time a realistic extended jet model has been used to constrain the dynamical and structural properties of a large sample of blazars by fitting to their spectra. We include the fits to the remaining 32 SEDs not fitted in Chapter 5 and the fitted parameter values for all 38 blazars (plus the 4 quasi-simultaneous HSP BL Lacs from \cite{2012MNRAS.422L..48P} fitted in Chapter 5) in Appendix A.

\section{Results}



\begin{figure*}
	\centering
		\subfloat[]{ \includegraphics[width=12cm, clip=true, trim=2cm 1cm 1cm 2cm]{corr1colmod.pdf} }
\\
		\subfloat[]{ \includegraphics[width=12cm, clip=true, trim=2cm 1cm 1cm 2cm]{corr2colmod.pdf} }	
		
	\caption{The results of fitting our model to all 38 blazars with simultaneous multiwavelength spectra and redshifts and the 4 quasi-simultaneous HSP BL Lac SEDs from Chapter 5. Figure a shows the distance of the jet transition region plotted against the jet power for all fits. We see a clear correlation between the jet power and radius of the transition region as suggested in our previous work. BL Lacs have systematically smaller radius transition regions than FSRQs, with an approximately linear correlation between the two as illustrated by the dashed lines. We have highlighted the two outliers to the relation, Markarian 421 and 3C273. We argue that these two blazars are atypical since Mkn421 is one of the closest known blazars and 3C273 is the one of the most powerful (and seems to be misaligned). Figure b shows the maximum bulk Lorentz factor plotted against the radius of the transition region. We see that the bulk Lorentz factor is systematically larger for FSRQs than BL Lacs and increases with the distance over which the jet accelerates as we expect. }
	\label{corr}
\end{figure*}

\begin{figure*}
	\centering
		\subfloat[]{ \includegraphics[height=5.5cm, clip=true, trim=2cm 1cm 1cm 2cm]{boxplotEddmod.pdf} }
		\subfloat[]{ \includegraphics[height=5.5cm, clip=true,  trim=2cm 2cm 1cm 2cm]{boxplotjetlengthmod.pdf} }	
	\caption{The distribution of fractional Eddington luminosity and the distance to the jet transition region under the assumption of a constant black hole mass of $5\times 10^{8}M_{\odot}$ for all 38 blazars with simultaneous observations. Figure a shows a clear dichotomy in the fractional Eddington luminosity between BL Lacs and FSRQs suggestive of two accretion modes. Figure b shows that the accelerating transition region extends out to larger distances in FSRQs than BL Lacs, this could be responsible for the different maximum bulk Lorentz factors shown in Figure \ref{corr}b. }
	\label{distributions}
\end{figure*}

\begin{figure*}
	\centering
		\subfloat{ \includegraphics[width=12cm, clip=true, trim=2cm 1cm 1cm 2cm]{corr3colmod.pdf} }
		
	\caption{ The inferred black hole mass of the fits plotted against jet power assuming the transition region occurs at a distance of $10^{5}r_{s}$ as in M87. The range of black hole masses is compatible with that found from large galaxy surveys ($10^{7}$--$10^{10}M_{\odot}$). We naturally find a linear relation between jet power and the radius of the transition region if we assume all blazars are accreting at a similar Eddington fraction $0.01-0.1L_{Edd}$.}
	\label{corr3}
\end{figure*}

We show the key results of fitting this model to spectra of the 38 blazars with simultaneous multiwavelength observations and the 4 HSP BL Lacs from \cite{2012MNRAS.422L..48P} (fitted in Chapter 5) in Figure \ref{corr}. We find an approximately linear relation between the total jet power and the radius where the jet transitions from parabolic to conical, stops accelerating and first comes into equipartition. The results also confirm that the blazar population can be divided into FSRQs with the highest power jets and BL Lacs with low power jets (\cite{2008MNRAS.387.1669G} and \cite{2009MNRAS.396L.105G}). 

We also find a clear correlation between the radius of the jet at the transition region and the maximum bulk Lorentz factor of the jet shown in Figure \ref{corr}b. This is very significant for two reasons: firstly, it has long been thought from unification that FSRQ and BL Lac type blazars correspond to FRII and FRI type jets observed at small angles to the line of sight (\cite{1995PASP..107..803U}) and secondly, from theoretical and numerical work, we expect jets with larger bulk Lorentz factors to accelerate over larger distances, with the precise form of the dependence giving us information about the geometry of the magnetic field lines in the accelerating region of the jet (\cite{2003ApJ...596.1080V}, \cite{2006MNRAS.367..375B} and \cite{2009MNRAS.394.1182K}). For the first time we see strong evidence confirming both these ideas from systematically studying the SEDs of a large sample of blazars. 

We have fitted these blazar spectra by eye, however, we are confident of the results in Figure \ref{corr}a, since they are supported by simple, physical arguments. We find an absence of low power blazars with large emitting regions and high power blazars with small emitting regions. This is to be expected because low power blazars with large emitting regions would have very low magnetic field strengths at the transition region. Their peak synchrotron and SSC frequencies would be very low and their SSC emission would be very weak, making them undetectable with current $\gamma$-ray observations. Low power blazars are observed to have high peak frequencies of emission, with no synchrotron break visible at low frequencies. This is not compatible with low power blazars with large transition regions. High power blazars with small radius transition regions would produce spectra with synchrotron break frequencies occurring at too high frequencies (see Figure \ref{Ch3fig:1}b). In addition SSC emission would dominate their $\gamma$-ray emission and this would not allow them to become Compton-dominant due to the self-limiting nature of SSC emission. For these reasons we are confident in the results shown in Figure \ref{corr}.

We find that we are only able to fit the quiescent gamma ray emission from FSRQs if the jets scatter CMB photons at large distances along the jets and the jets remain relativistic until kpc scales (as in FRII jets, \cite{1974MNRAS.169..395B}). The inverse-Compton emission of most BL Lacs requires a dominant SSC component to match their spectra and we find that they do not have such large bulk Lorentz factors as FSRQs. In addition, we notice that the radio spectra of FSRQs in the sample are systematically steeper than the flat radio spectra of BL Lacs. We find that this requires that FSRQ jets become more particle dominated at large distances past the transition region while BL Lac jets remain close to equipartition along the jet. This distinction could be responsible for the morphological differences between FRII and FRI jets (where a magnetised jet can be susceptible to additional MHD instabilities such as the kink instability \cite{2012ApJ...757...16M}). 

We expect most FSRQs to be associated with FRII jets and most BL Lacs to be associated with FRI type jets because it is known that the jet power is a strong indicator of the jet morphology (\cite{1974MNRAS.167P..31F}). It is thought that FRII jets need to be sufficiently powerful not to be decelerated by their environment and become subsonic on pc scales. This has been used to predict the FRI/FRII divide in power (\cite{1995ApJS..101...29B}). We do not suggest that the blazar classification, based on line widths, is the direct cause of the jet morphology (since line widths are clearly an indirect measurement of the accretion process) but that it provides a good indicator of the jet power and thereby the FR classification of the jet. Figure \ref{distributions}a shows that overall the blazar classification corresponds to high and low power jets, however, there is clearly an overlapping region where the blazar classification loses its descriminating power. This is analogous to evidence that high and low excitation radio galaxies (HERGs and LERGs) are related to the accretion mode, with HERGs having high Eddington accretion rates and radiatively efficient thin discs and LERGs corresponding to a sub-Eddington radiatively inefficient mode (\cite{2009MNRAS.396.1929H}). There is also evidence for the broad association of HERGs with FRII type jets and LERGs with FRI jets, however, there also exist a small proportion of FRII LERGs and FRI LERGs (\cite{2007MNRAS.376.1849H}). It seems likely that choosing a particular observational classification for AGN/blazars which broadly divides the population by accretion power leads to an association of the classification with FR type. It is important to remember, however, that the observational classification is not the primary, causal variable but could still be a good indirect indicator of the jet power and environment. This leads to regions in which the relation between observational and FR classification breaks down. We find that our results provide strong evidence for the association of most FSRQs with FRII jets and most BL Lacs with FRI jets. We have also found evidence for the distinct physical properties of FRI and FRII jets which could lead to their morphological definitions.

Besides constraining the dependence of the jet structure and dynamics on blazar parameters in unprecedented detail, we can also use our model to understand the physics behind the blazar sequence (\cite{1998MNRAS.299..433F}) for the first time. We find a linear relation between the jet power and the radius of the transition region which dominates the optically thin synchrotron emission in our jet. The transition region dominates the optically thin synchrotron emission because this is the point at which the plasma first comes into equipartition (a plasma with a fixed total energy radiates synchrotron power most efficiently close to equipartition) and has its maximum Lorentz factor. Low power blazars have smaller radius transition regions than high power blazars and since $B^{2}\propto W_{j}/(R^{2} \gamma_{\m{bulk}}^2)$ the magnetic field strength is larger in BL Lacs compared to FSRQs. This results naturally in the anticorrelation between peak synchrotron frequency and jet power seen in the blazar sequence because the peak synchrotron frequency depends linearly on the magnetic field strength, which is larger in BL Lacs than FSRQs.

Furthermore, we find that in low power blazars with compact transition regions and high magnetic field strengths the number density of synchrotron photons is large and so the inverse-Compton emission is due to scattering high frequency SSC photons. The Compton-catastrophe prevents SSC blazars from becoming significantly Compton-dominant as required by many FSRQs. Meanwhile high power blazars with higher bulk Lorentz factors and larger transition regions with lower magnetic field strengths emit less power through synchrotron emission and so the number density of synchrotron photons is too low to reproduce their gamma-ray emission via SSC. The large bulk Lorentz factor allows them to scatter low energy CMB photons at large distances along the jet resulting in their low inverse-Compton peak frequencies and Compton dominance. This coherent picture of a changing transition region radius and bulk Lorentz factor allows us to understand the structural and dynamic changes in jets which produce the blazar sequence as suggested in Chapters 4 and 5.

We can go one step further and motivate this emerging jet paradigm by using the results of black hole mass estimates. \cite{2013ApJ...764..135S} found that BL Lacs have black hole masses with a range $10^{8.5}-10^{9}M_{\odot}$ while FSRQs had a similar range $ 10^{8}-10^{9}M_{\odot}$ with slightly lower masses on average (\cite{2012ApJ...748...49S}). While individual mass estimates are quite uncertain these indirect mass estimates indicate that BL Lac and FSRQ masses are similar with BL Lacs being slightly larger (though less well constrained due to a lack of strong emission lines). Taking into account the similar black hole masses of FSRQs and BL Lacs and, for simplicity, assuming a constant fiducial mass of $5\times 10^{8}M_{\odot}$ we can plot the distribution of fractional Eddington luminosity as a function of the jet power of a blazar and also the distance at which the transition region occurs in their jets. It is very interesting to find that the BL Lacs and FSRQs naturally split into the bimodal distribution in these quantities shown in Figure \ref{distributions}. BL Lacs have low Eddington accretion rates $\sim10^{-3}L_{Edd}$ while FSRQs have larger Eddington accretion rates $0.1-1L_{Edd}$. This is exactly the behaviour suggested by X-ray binary jets in which accreting black holes produce low power, mildly relativistic jets in a radiatively inefficient sub Eddington state, while the transition from this low state to a thin radiatively efficient disc with a high accretion rate temporarily produces a highly relativistic jet (\cite{2004MNRAS.355.1105F}). 

We propose that our results offer the first solid evidence for this scenario in blazars by fitting a realistic physically rigorous model for jet emission to accurately estimate the jet power by fitting to radio observations. We find that FSRQs have high accretion rates around the Eddington luminosity, producing fast jets which accelerate over large distances and become particle dominated at large distances whilst maintaining their bulk Lorentz factors (characteristic of FRII jets). BL Lacs represent the X-ray binary low/hard state with a radiatively inefficient disc accreting at a low Eddington fraction and producing slower jets which accelerate over smaller distances. They remain magnetised and close to equipartition at large distances, breaking up due to instabilities characteristic of FRI type jets. The different bulk Lorentz factors are likely to be related to the different accretion modes in the two cases, with a hot, thick, radiatively inefficient accretion disc in BL Lacs entraining more disc material at the base of the jet and resulting in a larger mass loading and lower final bulk Lorentz factor than in FSRQs whose thin discs are radiatively efficient.

Alternatively, if we ignore the results of indirect black hole mass estimates in blazars due to their unreliability, we must consider a different scenario. If all blazar jets scale only with black hole mass (as assumed in MHD simulations and theoretical work) we can infer the black hole mass by constraining the transition region to occur at $10^{5}r_{s}$ in all jets (as in M87), shown in Figure \ref{corr3}. In this case we find black hole masses in the range $10^{7}-10^{10}M_{\odot}$ consistent with galaxy surveys. We also find that BL Lacs have smaller black hole masses than FSRQs and the linear relation between jet power and transition region radius means that all these blazars have approximately the same Eddington accretion fraction between $0.01-0.1L_{Edd}$. The scenario of a universal jet structure which scales linearly with black hole mass is appealing for its simplicity and is assumed in current state of the art GRMHD jet simulations (for example \cite{2009MNRAS.394.1182K}, \cite{2010ApJ...711...50T} and \cite{2012MNRAS.423.3083M}). There are two problems with this scenario however: the first is that this trend is not consistent with indirect measurements of black hole masses and the second is that this scenario doesn't explain the difference we find in bulk Lorentz factors between BL Lacs and FSRQs. Also, this does not tie in with the connection between accretion mode state and jet production from X-ray binaries or the expected correspondence of FRI and FRII jets to BL Lacs and FSRQs as we expect from unification. For these reasons we currently favour a bimodal accretion mode between BL Lacs and FSRQs linked to the FRI/FRII dichotomy. Obviously, the most direct way in which to settle this would be through a comparison to reliable black hole mass measurements for blazars. 

\section{Summary}

In this Chapter we have shown that our jet model with a magnetically dominated accelerating parabolic base transitioning to a slowly decelerating conical jet is able to fit to observations of blazar jets with unprecedented detail across all frequencies. This offers support for the emerging picture of jets motivated by observations and simulations. We find that in fitting to a large sample of blazar spectra we are able to constrain dynamic and structural properties of blazar jets. Our two main results are: the discovery of a linear correlation between the radius of the transition region of the jet and the jet power; a relation between the maximum bulk Lorentz factor and the distance over which the jet accelerates before reaching equipartition. These results allow us to understand the physical origin of the blazar sequence for the first time but also offer evidence for an accretion mode dichotomy in AGN analogous to that observed in X-ray binary systems and consistent with a correspondence between BL Lac and FSRQs, FRI and FRII jet properties and the mode of accretion.
\newpage
\section{Appendix A}

\begin{figure*}
	\centering
		\subfloat[J0137]{ \includegraphics[width=8cm, clip=true, trim=1.5cm 1cm 2.5cm 1.5cm]{J0137.pdf} }
		\subfloat[J0210]{ \includegraphics[width=8cm, clip=true, trim=1.5cm 1cm 2.5cm 1.5cm]{J0210.pdf} }	
\\
\subfloat[J0229]{ \includegraphics[width=8cm, clip=true, trim=1.5cm 1cm 2.5cm 1.5cm]{J0229.pdf} }
		\subfloat[J0238.4]{ \includegraphics[width=8cm, clip=true, trim=1.5cm 1cm 2.5cm 1.5cm]{J02384.pdf} }	
\\
\subfloat[J0238.6]{ \includegraphics[width=8cm, clip=true, trim=1.5cm 1cm 2.5cm 1.5cm]{J02386.pdf} }
\subfloat[J0349]{ \includegraphics[width=8cm, clip=true, trim=1.5cm 1cm 2.5cm 1.5cm]{J0349.pdf} }	
		
	\caption{The fits to the SEDs of the remaining 32 blazars with simultaneous multiwavelength observations and redshifts from \cite{2010ApJ...716...30A}, not fitted in Chapter 5. The model is able to fit very well to all of the spectra including radio observations.}
\label{fig51}
\end{figure*}

\begin{figure*}
	\centering
		
		\subfloat[J0423]{ \includegraphics[width=8cm, clip=true, trim=1.5cm 1cm 2.5cm 1.5cm]{J0423.pdf} }
		\subfloat[J0457]{ \includegraphics[width=8cm, clip=true, trim=1.5cm 1cm 2.5cm 1.5cm]{J0457.pdf} }
\\	
\subfloat[J0507]{ \includegraphics[width=8cm, clip=true, trim=1.5cm 1cm 2.5cm 1.5cm]{J0507.pdf} }
\subfloat[J0531]{ \includegraphics[width=8cm, clip=true, trim=1.5cm 1cm 2.5cm 1.5cm]{J0531.pdf} }	
\\
\subfloat[J0538]{ \includegraphics[width=8cm, clip=true, trim=1.5cm 1cm 2.5cm 1.5cm]{J0538.pdf} }
\subfloat[J0730]{ \includegraphics[width=8cm, clip=true, trim=1.5cm 1cm 2.5cm 1.5cm]{J0730.pdf} }	
\caption{}
		
\label{fig52}

\end{figure*}

\begin{figure*}
	\centering
		\subfloat[J0921]{ \includegraphics[width=8cm, clip=true, trim=1.5cm 1cm 2.5cm 1.5cm]{J0921.pdf} }
\subfloat[J1057]{ \includegraphics[width=8cm, clip=true, trim=1.5cm 1cm 2.5cm 1.5cm]{J1057.pdf} }	
\\
\subfloat[J1159]{ \includegraphics[width=8cm, clip=true, trim=1.5cm 1cm 2.5cm 1.5cm]{J1159.pdf} }
		\subfloat[J1221]{ \includegraphics[width=8cm, clip=true, trim=1.5cm 1cm 2.5cm 1.5cm]{J1221.pdf} }			
\\
\subfloat[J1229]{ \includegraphics[width=8cm, clip=true, trim=1.5cm 1cm 2.5cm 1.5cm]{J1229.pdf} }	
\subfloat[J1256]{ \includegraphics[width=8cm, clip=true, trim=1.5cm 1cm 2.5cm 1.5cm]{J1256.pdf} }
\caption{}	
		
\label{fig53}

\end{figure*}

\begin{figure*}
	\centering
\subfloat[J1310]{ \includegraphics[width=8cm, clip=true, trim=1.5cm 1cm 2.5cm 1.5cm]{J1310.pdf} }	
\subfloat[J1457]{ \includegraphics[width=8cm, clip=true, trim=1.5cm 1cm 2.5cm 1.5cm]{J1457.pdf} }		
\\
\subfloat[J1504]{ \includegraphics[width=8cm, clip=true, trim=1.5cm 1cm 2.5cm 1.5cm]{J1504.pdf} }	
		\subfloat[J1512]{ \includegraphics[width=8cm, clip=true, trim=1.5cm 1cm 2.5cm 1.5cm]{J1512.pdf} }		
\\
\subfloat[J1522]{ \includegraphics[width=8cm, clip=true, trim=1.5cm 1cm 2.5cm 1.5cm]{J1522.pdf} }	
\subfloat[Mkn501]{ \includegraphics[width=8cm, clip=true, trim=1.5cm 1cm 2.5cm 1.5cm]{Mkn501.pdf} }		
\caption{}
		

\label{fig54}

\end{figure*}

\begin{figure*}
	\centering
\subfloat[J1719]{ \includegraphics[width=8cm, clip=true, trim=1.5cm 1cm 2.5cm 1.5cm]{J1719.pdf} }
\subfloat[J1849]{ \includegraphics[width=8cm, clip=true, trim=1.5cm 1cm 2.5cm 1.5cm]{J1849.pdf} }				
\\
\subfloat[J2000]{ \includegraphics[width=8cm, clip=true, trim=1.5cm 1cm 2.5cm 1.5cm]{J2000.pdf} }
\subfloat[J2143]{ \includegraphics[width=8cm, clip=true, trim=1.5cm 1cm 2.5cm 1.5cm]{J2143.pdf} }		
\\
\subfloat[BLLac]{ \includegraphics[width=8cm, clip=true, trim=1.5cm 1cm 2.5cm 1.5cm]{BLLac.pdf} }	
\subfloat[J2254]{ \includegraphics[width=8cm, clip=true, trim=1.5cm 1cm 2.5cm 1.5cm]{J2254.pdf} }		
\caption{}		

\label{fig55}

\end{figure*}

\begin{figure*}
	\centering
		\subfloat[J2327]{ \includegraphics[width=8cm, clip=true, trim=1.5cm 1cm 2.5cm 1.5cm]{J2327.pdf} }	
		\subfloat[J2345]{ \includegraphics[width=8cm, clip=true, trim=1.5cm 1cm 2.5cm 1.5cm]{J2345.pdf} }	
\caption{}	
\label{fig56}

\end{figure*}
\newpage

\begin{sidewaystable}
\centering
\begin{tabular}{| c | c | c | c | c | c | c | c | c | c | c | c | c | c | c | c |}
\hline
Blazar & $W_{j}$(W) & $L$(m) & $ E_{\m{max}}$(MeV) & $\alpha$  & $\theta_{\m{observe}}$ & $\gamma_{\m{max}}$ & $\gamma_{\m{min}}$ & $ L_{\m{acc}}$(W) & $ R_{T}$(m) & $ B_{T}$(T)& $M(M_{\odot})$  \\ \hline 
J0035 & $5.0 \times 10^{37}$ & $10^{20}$ & $40.6$ & $1.3$ & $1^{0}$ & $14$ & $10$ & $1.67\times 10^{38}$ & $2.70\times 10^{14}$ & $5.91\times 10^{-5}$ & $7.69\times 10^{7}$ \\ \hline
J0137 & $7.06\times 10^{38}$ & $1\times 10^{21}$ & $22.8$ & $2.35$ & $1^{0}$ & $27$ & $16$ & $2.5\times 10^{38}$ & $1.21\times 10^{16}$ & $2.58\times 10^{-6}$ & $3.44\times 10^{9}$ \\ \hline
J0210 & $7.78\times 10^{38}$ & $2\times 10^{21}$ & $5.11$ & $2.01$ & $1^{0}$ & $38$ & $20$ & $4.27\times 10^{38}$ & $9.76\times 10^{15}$ & $2.38\times 10^{-6}$ & $2.78\times 10^{9}$ \\ \hline
J0222 & $1.04\times 10^{38}$ & $5\times 10^{20}$ & $16.2$ & $1.6$ & $1^{0}$ & $12$ & $8$ & $1.67\times 10^{38}$ & $1.47\times 10^{14}$ & $0.000184$ & $4.17\times 10^{7}$ \\ \hline
J0229 & $7\times 10^{38}$ & $1\times 10^{21}$ & $8.1$ & $1.9$ & $1^{0}$ & $40$ & $30$ & $4.17\times 10^{38}$ & $1.23\times 10^{16}$ & $1.7\times 10^{-6}$ & $3.5\times 10^{9}$ \\ \hline
J0238.4 & $1.2\times 10^{39}$ & $1\times 10^{21}$ & $8.1$ & $2.15$ & $1.2^{0}$ & $25$ & $15$ & $3.42\times 10^{38}$ & $3.27\times 10^{16}$ & $1.34\times 10^{-6}$ & $9.29\times 10^{9}$ \\ \hline
J0238.6 & $1.71\times 10^{39}$ & $1\times 10^{21}$ & $14.4$ & $2.01$ & $1^{0}$ & $38$ & $25$ & $5.7\times 10^{38}$ & $5.98\times 10^{15}$ & $5.78\times 10^{-6}$ & $1.69\times 10^{9}$ \\ \hline
J0349 & $1.67\times 10^{39}$ & $1\times 10^{21}$ & $6.74$ & $1.45$ & $1^{0}$ & $30$ & $8$ & $8.33\times 10^{38}$ & $1.48\times 10^{16}$ & $2.91\times 10^{-6}$ & $4.21\times 10^{9}$ \\ \hline
J0423 & $1\times 10^{39}$ & $2\times 10^{21}$ & $4.06$ & $2.11$ & $1^{0}$ & $30$ & $18$ & $1.99\times 10^{38}$ & $1.41\times 10^{16}$ & $2.37\times 10^{-6}$ & $4.01\times 10^{9}$ \\ \hline
J0457 & $8.5\times 10^{38}$ & $1\times 10^{21}$ & $8.1$ & $1.85$ & $1^{0}$ & $33$ & $20$ & $3.33\times 10^{38}$ & $3.52\times 10^{16}$ & $7.95\times 10^{-7}$ & $1\times 10^{10}$ \\ \hline
J0507 & $1.85\times 10^{37}$ & $2\times 10^{21}$ & $32.2$ & $1.5$ & $2^{0}$ & $16$ & $10$ & $8.55\times 10^{37}$ & $4.41\times 10^{13}$ & $0.000193$ & $1.26\times 10^{7}$ \\ \hline
J0531 & $2.17\times 10^{39}$ & $2\times 10^{21}$ & $2.87$ & $1.6$ & $1^{0}$ & $28$ & $13$ & $1.39\times 10^{39}$ & $4.40\times 10^{16}$ & $1.2\times 10^{-6}$ & $1.25\times 10^{10}$ \\ \hline
J0537 & $8.0\times 10^{37}$ & $1\times 10^{21}$ & $102$ & $1.75$ & $1.5^{0}$ & $12$ & $6$ & $1.25\times 10^{35}$ & $5.41\times 10^{14}$ & $4.36\times 10^{-5}$ & $1.54\times 10^{8}$  \\ \hline
J0538 & $1.78\times 10^{39}$ & $1\times 10^{21}$ & $10.2$ & $2.2$ & $1^{0}$ & $40$ & $22$ & $6.84\times 10^{38}$ & $2.20\times 10^{16}$ & $1.52\times 10^{-6}$ & $6.25\times 10^{9}$ \\ \hline
J0630 & $2.1\times 10^{38}$ & $1\times 10^{20}$ & $81$ & $1.3$ & $1$ & $14$ & $10$ & $1.25\times 10^{35}$ & $1.35\times 10^{15}$ & $2.42\times 10^{-5}$ & $3.85\times 10^{8}$ \\ \hline
J0730 & $2.14\times 10^{39}$ & $1\times 10^{21}$ & $4.55$ & $1.7$ & $1^{0}$ & $26$ & $15$ & $1.08\times 10^{39}$ & $3.06\times 10^{16}$ & $1.84\times 10^{-6}$ & $8.7\times 10^{9}$ \\ \hline
J0855 & $1.56\times 10^{38}$ & $5\times 10^{20}$ & $5.11$ & $1.63$ & $1^{0}$ & $8$ & $6$ & $8.33\times 10^{36}$ & $4.05\times 10^{14}$ & $0.000122$ & $1.15\times 10^{8}$ \\ \hline
J0921 & $1.91\times 10^{39}$ & $1\times 10^{21}$ & $8.1$ & $2.1$ & $1^{0}$ & $30$ & $18$ & $8.55\times 10^{38}$ & $1.30\times 10^{16}$ & $3.53\times 10^{-6}$ & $3.71\times 10^{9}$ \\ \hline
J1015 & $2.41\times 10^{37}$ & $1\times 10^{21}$ & $32.2$ & $1.5$ & $3.5^{0}$ & $10$ & $3$ & $2.5\times 10^{37}$ & $5.85\times 10^{13}$ & $0.000266$ & $1.66\times 10^{7}$ \\ \hline
J1057 & $9.41\times 10^{38}$ & $1\times 10^{21}$ & $4.06$ & $2.1$ & $1^{0}$ & $26$ & $20$ & $5.7\times 10^{37}$ & $1.11\times 10^{16}$ & $3.36\times 10^{-6}$ & $3.16\times 10^{9}$ \\ \hline
J1159 & $5.33\times 10^{38}$ & $2\times 10^{21}$ & $3.45$ & $1.95$ & $1^{0}$ & $30$ & $15$ & $1.14\times 10^{38}$ & $7.34\times 10^{15}$ & $3.31\times 10^{-6}$ & $2.09\times 10^{9}$ \\ \hline
J1221 & $1.71\times 10^{37}$ & $1\times 10^{21}$ & $32.2$ & $1.75$ & $2^{0}$ & $19$ & $10$ & $1.14\times 10^{37}$ & $2.22\times 10^{15}$ & $3.11\times 10^{-6}$ & $6.31\times 10^{8}$ \\ \hline
J1229 & $7.5\times 10^{39}$ & $1\times 10^{21}$ & $3.22$ & $1.2$ & $8.5^{0}$ & $12$ & $8$ & $1.97\times 10^{39}$ & $3.17\times 10^{15}$ & $7.22\times 10^{-5}$ & $9\times 10^{8}$ \\ \hline
J1256 & $1.64\times 10^{39}$ & $1\times 10^{21}$ & $3.22$ & $2.1$ & $1^{0}$ & $37$ & $18$ & $1.99\times 10^{38}$ & $1.76\times 10^{16}$ & $1.97\times 10^{-6}$ & $5.01\times 10^{9}$ \\ \hline

\end{tabular}
\caption{The values of the physical parameters used in the fits from this Chapter (shown in Figures $\ref{fig51}$--\ref{fig56}) and Chapter 5.}
\label{tab51}

\end{sidewaystable}

\begin{sidewaystable}
\centering
\begin{tabular}{| c | c | c | c | c | c | c | c | c | c | c | c | c | c | c | c |}
\hline

Blazar & $W_{j}$(W) & $L$(m) & $ E_{\m{max}}$(MeV) & $\alpha$  & $\theta_{\m{observe}}$ & $\gamma_{\m{max}}$ & $\gamma_{\m{min}}$ & $ L_{\m{acc}}$(W) & $ R_{T}$(m) & $ B_{T}$(T)& $M(M_{\odot})$  \\ \hline 
J1310 & $1.5\times 10^{39}$ & $1\times 10^{21}$ & $2.56$ & $1.95$ & $1^{0}$ & $50$ & $30$ & $2.28\times 10^{38}$ & $5.01\times 10^{15}$ & $4.89\times 10^{-6}$ & $1.43\times 10^{9}$ \\ \hline
J1312 & $2.3\times 10^{38}$ & $1\times 10^{21}$ & $81$ & $1.6$ & $1.2^{0}$ & $10$ & $6$ & $2.5\times 10^{34}$ & $1.62\times 10^{15}$ & $2.96\times 10^{-5}$ & $4.62\times 10^{8}$ \\ \hline
J1457 & $1.17\times 10^{39}$ & $1\times 10^{21}$ & $14.4$ & $2.05$ & $1^{0}$ & $36$ & $25$ & $5.7\times 10^{38}$ & $2.54\times 10^{16}$ & $1.18\times 10^{-6}$ & $7.22\times 10^{9}$ \\ \hline
J1504 & $2.04\times 10^{39}$ & $1\times 10^{21}$ & $17.3$ & $1.85$ & $1^{0}$ & $42$ & $16$ & $1.5\times 10^{39}$ & $5.92\times 10^{16}$ & $5.72\times 10^{-7}$ & $1.69\times 10^{10}$ \\ \hline
J1512 & $4.62\times 10^{38}$ & $2\times 10^{21}$ & $3.22$ & $1.9$ & $1^{0}$ & $45$ & $35$ & $7.69\times 10^{37}$ & $1.47\times 10^{16}$ & $1.03\times 10^{-6}$ & $4.18\times 10^{9}$ \\ \hline
J1522 & $6.52\times 10^{38}$ & $1\times 10^{21}$ & $5.73$ & $1.65$ & $1^{0}$ & $36$ & $18$ & $1.08\times 10^{38}$ & $3.12\times 10^{16}$ & $7.18\times 10^{-7}$ & $8.89\times 10^{9}$ \\ \hline
J1719 & $3.39\times 10^{37}$ & $1\times 10^{21}$ & $8.1$ & $2.2$ & $1^{0}$ & $45$ & $25$ & $1.42\times 10^{36}$ & $2.22\times 10^{15}$ & $1.85\times 10^{-6}$ & $6.31\times 10^{8}$ \\ \hline
J1751 & $2.08\times 10^{38}$ & $2\times 10^{21}$ & $4.06$ & $1.98$ & $1^{0}$ & $34$ & $18$ & $3.33\times 10^{37}$ & $6.45\times 10^{15}$ & $2.08\times 10^{-6}$ & $1.83\times 10^{9}$ \\ \hline
J1849 & $6.25\times 10^{38}$ & $1\times 10^{21}$ & $8.1$ & $2.2$ & $1^{0}$ & $40$ & $25$ & $8.55\times 10^{37}$ & $6.33\times 10^{15}$ & $3.13\times 10^{-6}$ & $1.79\times 10^{9}$ \\ \hline
J2000 & $2.8\times 10^{36}$ & $1\times 10^{21}$ & $128$ & $1.6$ & $4^{0}$ & $8$ & $4$ & $1.14\times 10^{37}$ & $3.52\times 10^{13}$ & $0.000188$ & $1\times 10^{7}$ \\ \hline
J2143 & $2.5\times 10^{37}$ & $5\times 10^{20}$ & $3.08$ & $1.45$ & $3^{0}$ & $10$ & $6$ & $1.14\times 10^{37}$ & $5.44\times 10^{13}$ & $0.000291$ & $1.55\times 10^{7}$ \\ \hline
J2158 & $1.55\times 10^{37}$ & $1\times 10^{20}$ & $51.1$ & $1.7$ & $2^{0}$ & $15$ & $7$ & $2.5\times 10^{37}$ & $1.01\times 10^{14}$ & $8.2\times 10^{-5}$ & $2.87\times 10^{7}$ \\ \hline
J2254 & $4.44\times 10^{39}$ & $3\times 10^{21}$ & $6.43$ & $2.05$ & $0.8^{0}$ & $60$ & $35$ & $2.28\times 10^{38}$ & $2.20\times 10^{16}$ & $1.6\times 10^{-6}$ & $6.25\times 10^{9}$ \\ \hline
J2327 & $1.23\times 10^{39}$ & $3\times 10^{21}$ & $1.81$ & $1.5$ & $0.8^{0}$ & $50$ & $32$ & $7.12\times 10^{38}$ & $3.98\times 10^{15}$ & $5.58\times 10^{-6}$ & $1.13\times 10^{9}$ \\ \hline
J2345 & $5\times 10^{38}$ & $2\times 10^{21}$ & $8.1$ & $1.95$ & $1.3^{0}$ & $50$ & $35$ & $5.7\times 10^{37}$ & $1.08\times 10^{16}$ & $1.3\times 10^{-6}$ & $3.06\times 10^{9}$ \\ \hline
Mkn421 & $6\times 10^{36}$ & $3\times 10^{20}$ & $338$ & $1.55$ & $3^{0}$ & $12$ & $9$ & $2.5\times 10^{36}$ & $2.22\times 10^{15}$ & $2.91\times 10^{-6}$ & $6.31\times 10^{8}$ \\ \hline
Mkn501 & $6.5\times 10^{36}$ & $1\times 10^{20}$ & $228$ & $1.68$ & $6.5^{0}$ & $9$ & $2$ & $8.55\times 10^{36}$ & $1.11\times 10^{14}$ & $8.06\times 10^{-5}$ & $3.16\times 10^{7}$ \\ \hline
BL Lac & $9\times 10^{36}$ & $5\times 10^{20}$ & $8.1$ & $1.95$ & $3^{0}$ & $8$ & $5$ & $8.33\times 10^{36}$ & $4.43\times 10^{13}$ & $0.000268$ & $1.26\times 10^{7}$ \\ \hline

\end{tabular}

\end{sidewaystable}

==> Paper 5/Chapter5.tex <==
\chapter{Understanding the physics behind the blazar population}
\ifpdf
    \graphicspath{{Chapter5/Chapter5Figs/PNG/}{Chapter5/Chapter5Figs/PDF/}{Chapter5/Chapter5Figs/}}
\else
    \graphicspath{{Chapter5/Chapter5Figs/EPS/}{Chapter5/Chapter5Figs/}}
\fi

This is the concluding Chapter of my work modelling blazars. In this Chapter I use the model developed in Chapters 2-5 to fit to the remaining 32 blazars with simultaneous multiwavelength spectra and redshifts available from the {\it Fermi} sample (\cite{2010ApJ...716...30A}). The model fits with unprecedented detail to all these blazars. I find strong empirical evidence for the predicted physical relation in Chapters 4 and 5; namely that the radius of the transition region and maximum bulk Lorentz factor increase with jet power. This is important since it provides an explanation for the basis of the blazar sequence.

I conclude that if black hole mass measurements can be believed, my results offer strong evidence for a scenario in which two accretion modes exist in blazars resulting in BL Lac and FSRQ type jets, analogous to the relationship between accretion mode and jet properties in X-ray binary systems. These sub-Eddington and Eddington accretion modes result in BL Lacs and FSRQs which have the expected properties of FRI and FRII jets observed close to the line of sight, as suggested by unification. These results are very exciting as they offer explanations and evidence for many long standing questions and hypotheses about blazars and AGN jets.

\section{Introduction}

%A fraction of supermassive black holes are observed to produce powerful, relativistic plasma jets. Blazars are the most extreme class of these jets in which we observe directly down the jet axis so the emission is strongly Doppler-boosted. These jets are created by the accretion of a magnetised plasma onto a spinning supermassive black hole at the centre of a galaxy. Jets are thought to be composed from electron positron pairs and are accelerated to within a fraction of the speed of light by the magnetic pressure gradient of a rotating, expanding helical magnetic field tied to the event horizon of a spinning black hole. 

%Jets are observed to emit radiation across the entire electromagnetic spectrum, however, existing compact emission models have been unable to constrain the structure and dynamics of these jets. Here we show an approximately linear relation exists between the jet power and the radius of the jet where the jet stops accelerating and first comes into equipartition. This is the first time that multifrequency observations including radio data have been successfully modelled for a large sample of blazars and we use these results to understand the physical reason behind the blazar sequence, which has long been a puzzle. We find evidence for a distinct difference in the properties of BL Lacs and FSRQs corresponding to FRI and FRII jets respectively and relate this to the bimodal accretion rate of BL Lacs and FSRQs if we assume both have similar black hole mass distributions.  

It has recently been observed that the jet in M87 has a parabolic base out to $10^{5}$ Schwarzschild radii becoming conical beyond this distance (\cite{2011arXiv1110.1793A}). This is consistent with state of the art numerical simulations which show the jet base starts magnetically dominated and accelerates in the parabolic region reaching a terminal bulk Lorentz factor at equipartition after which the jet becomes ballistic and conical (\cite{2006MNRAS.368.1561M}, \cite{2009MNRAS.394.1182K}, \cite{2010ApJ...711...50T} and \cite{2012MNRAS.423.3083M}). In this Chapter we use a model for the emission of a realistic jet motivated by and consistent with these recent observations and simulations in order to test this emerging picture of jets and to try to determine their properties.

We use the realistic extended jet model for emission from Chapters 2-5 (based on \cite{2012MNRAS.423..756P}, \cite{2013MNRAS.429.1189P}, \cite{2013MNRAS.431.1840P} and \cite{2013MNRASP4.}) to fit to the remaining 32 blazars with simultaneous multiwavelength observations and redshifts from the {\it Fermi} sample (\cite{2010ApJ...716...30A}). This model is the first to be able to simultaneously match the observations of blazars across all frequencies, including radio data, by considering the extended large scale structure of the jet. In being able to match the radio observations of jets we are able to tightly constrain the radius of the jet at the transition region by fitting the break frequency above which the synchrotron emission becomes optically thin (which sensitively depends on the radius at which the jet first approaches equipartition). This is the first time a realistic extended jet model has been used to constrain the dynamical and structural properties of a large sample of blazars by fitting to their spectra. We include the fits to the remaining 32 SEDs not fitted in Chapter 5 and the fitted parameter values for all 38 blazars (plus the 4 quasi-simultaneous HSP BL Lacs from \cite{2012MNRAS.422L..48P} fitted in Chapter 5) in Appendix A.

\section{Results}



\begin{figure*}
	\centering
		\subfloat[]{ \includegraphics[width=12cm, clip=true, trim=2cm 1cm 1cm 2cm]{corr1colmod.pdf} }
\\
		\subfloat[]{ \includegraphics[width=12cm, clip=true, trim=2cm 1cm 1cm 2cm]{corr2colmod.pdf} }	
		
	\caption{The results of fitting our model to all 38 blazars with simultaneous multiwavelength spectra and redshifts and the 4 quasi-simultaneous HSP BL Lac SEDs from Chapter 5. Figure a shows the distance of the jet transition region plotted against the jet power for all fits. We see a clear correlation between the jet power and radius of the transition region as suggested in our previous work. BL Lacs have systematically smaller radius transition regions than FSRQs, with an approximately linear correlation between the two as illustrated by the dashed lines. We have highlighted the two outliers to the relation, Markarian 421 and 3C273. We argue that these two blazars are atypical since Mkn421 is one of the closest known blazars and 3C273 is the one of the most powerful (and seems to be misaligned). Figure b shows the maximum bulk Lorentz factor plotted against the radius of the transition region. We see that the bulk Lorentz factor is systematically larger for FSRQs than BL Lacs and increases with the distance over which the jet accelerates as we expect. }
	\label{corr}
\end{figure*}

\begin{figure*}
	\centering
		\subfloat[]{ \includegraphics[height=5.5cm, clip=true, trim=2cm 1cm 1cm 2cm]{boxplotEddmod.pdf} }
		\subfloat[]{ \includegraphics[height=5.5cm, clip=true,  trim=2cm 2cm 1cm 2cm]{boxplotjetlengthmod.pdf} }	
	\caption{The distribution of fractional Eddington luminosity and the distance to the jet transition region under the assumption of a constant black hole mass of $5\times 10^{8}M_{\odot}$ for all 38 blazars with simultaneous observations. Figure a shows a clear dichotomy in the fractional Eddington luminosity between BL Lacs and FSRQs suggestive of two accretion modes. Figure b shows that the accelerating transition region extends out to larger distances in FSRQs than BL Lacs, this could be responsible for the different maximum bulk Lorentz factors shown in Figure \ref{corr}b. }
	\label{distributions}
\end{figure*}

\begin{figure*}
	\centering
		\subfloat{ \includegraphics[width=12cm, clip=true, trim=2cm 1cm 1cm 2cm]{corr3colmod.pdf} }
		
	\caption{ The inferred black hole mass of the fits plotted against jet power assuming the transition region occurs at a distance of $10^{5}r_{s}$ as in M87. The range of black hole masses is compatible with that found from large galaxy surveys ($10^{7}$--$10^{10}M_{\odot}$). We naturally find a linear relation between jet power and the radius of the transition region if we assume all blazars are accreting at a similar Eddington fraction $0.01-0.1L_{Edd}$.}
	\label{corr3}
\end{figure*}

We show the key results of fitting this model to spectra of the 38 blazars with simultaneous multiwavelength observations and the 4 HSP BL Lacs from \cite{2012MNRAS.422L..48P} (fitted in Chapter 5) in Figure \ref{corr}. We find an approximately linear relation between the total jet power and the radius where the jet transitions from parabolic to conical, stops accelerating and first comes into equipartition. The results also confirm that the blazar population can be divided into FSRQs with the highest power jets and BL Lacs with low power jets (\cite{2008MNRAS.387.1669G} and \cite{2009MNRAS.396L.105G}). 

We also find a clear correlation between the radius of the jet at the transition region and the maximum bulk Lorentz factor of the jet shown in Figure \ref{corr}b. This is very significant for two reasons: firstly, it has long been thought from unification that FSRQ and BL Lac type blazars correspond to FRII and FRI type jets observed at small angles to the line of sight (\cite{1995PASP..107..803U}) and secondly, from theoretical and numerical work, we expect jets with larger bulk Lorentz factors to accelerate over larger distances, with the precise form of the dependence giving us information about the geometry of the magnetic field lines in the accelerating region of the jet (\cite{2003ApJ...596.1080V}, \cite{2006MNRAS.367..375B} and \cite{2009MNRAS.394.1182K}). For the first time we see strong evidence confirming both these ideas from systematically studying the SEDs of a large sample of blazars. 

We have fitted these blazar spectra by eye, however, we are confident of the results in Figure \ref{corr}a, since they are supported by simple, physical arguments. We find an absence of low power blazars with large emitting regions and high power blazars with small emitting regions. This is to be expected because low power blazars with large emitting regions would have very low magnetic field strengths at the transition region. Their peak synchrotron and SSC frequencies would be very low and their SSC emission would be very weak, making them undetectable with current $\gamma$-ray observations. Low power blazars are observed to have high peak frequencies of emission, with no synchrotron break visible at low frequencies. This is not compatible with low power blazars with large transition regions. High power blazars with small radius transition regions would produce spectra with synchrotron break frequencies occurring at too high frequencies (see Figure \ref{Ch3fig:1}b). In addition SSC emission would dominate their $\gamma$-ray emission and this would not allow them to become Compton-dominant due to the self-limiting nature of SSC emission. For these reasons we are confident in the results shown in Figure \ref{corr}.

We find that we are only able to fit the quiescent gamma ray emission from FSRQs if the jets scatter CMB photons at large distances along the jets and the jets remain relativistic until kpc scales (as in FRII jets, \cite{1974MNRAS.169..395B}). The inverse-Compton emission of most BL Lacs requires a dominant SSC component to match their spectra and we find that they do not have such large bulk Lorentz factors as FSRQs. In addition, we notice that the radio spectra of FSRQs in the sample are systematically steeper than the flat radio spectra of BL Lacs. We find that this requires that FSRQ jets become more particle dominated at large distances past the transition region while BL Lac jets remain close to equipartition along the jet. This distinction could be responsible for the morphological differences between FRII and FRI jets (where a magnetised jet can be susceptible to additional MHD instabilities such as the kink instability \cite{2012ApJ...757...16M}). 

We expect most FSRQs to be associated with FRII jets and most BL Lacs to be associated with FRI type jets because it is known that the jet power is a strong indicator of the jet morphology (\cite{1974MNRAS.167P..31F}). It is thought that FRII jets need to be sufficiently powerful not to be decelerated by their environment and become subsonic on pc scales. This has been used to predict the FRI/FRII divide in power (\cite{1995ApJS..101...29B}). We do not suggest that the blazar classification, based on line widths, is the direct cause of the jet morphology (since line widths are clearly an indirect measurement of the accretion process) but that it provides a good indicator of the jet power and thereby the FR classification of the jet. Figure \ref{distributions}a shows that overall the blazar classification corresponds to high and low power jets, however, there is clearly an overlapping region where the blazar classification loses its descriminating power. This is analogous to evidence that high and low excitation radio galaxies (HERGs and LERGs) are related to the accretion mode, with HERGs having high Eddington accretion rates and radiatively efficient thin discs and LERGs corresponding to a sub-Eddington radiatively inefficient mode (\cite{2009MNRAS.396.1929H}). There is also evidence for the broad association of HERGs with FRII type jets and LERGs with FRI jets, however, there also exist a small proportion of FRII LERGs and FRI LERGs (\cite{2007MNRAS.376.1849H}). It seems likely that choosing a particular observational classification for AGN/blazars which broadly divides the population by accretion power leads to an association of the classification with FR type. It is important to remember, however, that the observational classification is not the primary, causal variable but could still be a good indirect indicator of the jet power and environment. This leads to regions in which the relation between observational and FR classification breaks down. We find that our results provide strong evidence for the association of most FSRQs with FRII jets and most BL Lacs with FRI jets. We have also found evidence for the distinct physical properties of FRI and FRII jets which could lead to their morphological definitions.

Besides constraining the dependence of the jet structure and dynamics on blazar parameters in unprecedented detail, we can also use our model to understand the physics behind the blazar sequence (\cite{1998MNRAS.299..433F}) for the first time. We find a linear relation between the jet power and the radius of the transition region which dominates the optically thin synchrotron emission in our jet. The transition region dominates the optically thin synchrotron emission because this is the point at which the plasma first comes into equipartition (a plasma with a fixed total energy radiates synchrotron power most efficiently close to equipartition) and has its maximum Lorentz factor. Low power blazars have smaller radius transition regions than high power blazars and since $B^{2}\propto W_{j}/(R^{2} \gamma_{\m{bulk}}^2)$ the magnetic field strength is larger in BL Lacs compared to FSRQs. This results naturally in the anticorrelation between peak synchrotron frequency and jet power seen in the blazar sequence because the peak synchrotron frequency depends linearly on the magnetic field strength, which is larger in BL Lacs than FSRQs.

Furthermore, we find that in low power blazars with compact transition regions and high magnetic field strengths the number density of synchrotron photons is large and so the inverse-Compton emission is due to scattering high frequency SSC photons. The Compton-catastrophe prevents SSC blazars from becoming significantly Compton-dominant as required by many FSRQs. Meanwhile high power blazars with higher bulk Lorentz factors and larger transition regions with lower magnetic field strengths emit less power through synchrotron emission and so the number density of synchrotron photons is too low to reproduce their gamma-ray emission via SSC. The large bulk Lorentz factor allows them to scatter low energy CMB photons at large distances along the jet resulting in their low inverse-Compton peak frequencies and Compton dominance. This coherent picture of a changing transition region radius and bulk Lorentz factor allows us to understand the structural and dynamic changes in jets which produce the blazar sequence as suggested in Chapters 4 and 5.

We can go one step further and motivate this emerging jet paradigm by using the results of black hole mass estimates. \cite{2013ApJ...764..135S} found that BL Lacs have black hole masses with a range $10^{8.5}-10^{9}M_{\odot}$ while FSRQs had a similar range $ 10^{8}-10^{9}M_{\odot}$ with slightly lower masses on average (\cite{2012ApJ...748...49S}). While individual mass estimates are quite uncertain these indirect mass estimates indicate that BL Lac and FSRQ masses are similar with BL Lacs being slightly larger (though less well constrained due to a lack of strong emission lines). Taking into account the similar black hole masses of FSRQs and BL Lacs and, for simplicity, assuming a constant fiducial mass of $5\times 10^{8}M_{\odot}$ we can plot the distribution of fractional Eddington luminosity as a function of the jet power of a blazar and also the distance at which the transition region occurs in their jets. It is very interesting to find that the BL Lacs and FSRQs naturally split into the bimodal distribution in these quantities shown in Figure \ref{distributions}. BL Lacs have low Eddington accretion rates $\sim10^{-3}L_{Edd}$ while FSRQs have larger Eddington accretion rates $0.1-1L_{Edd}$. This is exactly the behaviour suggested by X-ray binary jets in which accreting black holes produce low power, mildly relativistic jets in a radiatively inefficient sub Eddington state, while the transition from this low state to a thin radiatively efficient disc with a high accretion rate temporarily produces a highly relativistic jet (\cite{2004MNRAS.355.1105F}). 

We propose that our results offer the first solid evidence for this scenario in blazars by fitting a realistic physically rigorous model for jet emission to accurately estimate the jet power by fitting to radio observations. We find that FSRQs have high accretion rates around the Eddington luminosity, producing fast jets which accelerate over large distances and become particle dominated at large distances whilst maintaining their bulk Lorentz factors (characteristic of FRII jets). BL Lacs represent the X-ray binary low/hard state with a radiatively inefficient disc accreting at a low Eddington fraction and producing slower jets which accelerate over smaller distances. They remain magnetised and close to equipartition at large distances, breaking up due to instabilities characteristic of FRI type jets. The different bulk Lorentz factors are likely to be related to the different accretion modes in the two cases, with a hot, thick, radiatively inefficient accretion disc in BL Lacs entraining more disc material at the base of the jet and resulting in a larger mass loading and lower final bulk Lorentz factor than in FSRQs whose thin discs are radiatively efficient.

Alternatively, if we ignore the results of indirect black hole mass estimates in blazars due to their unreliability, we must consider a different scenario. If all blazar jets scale only with black hole mass (as assumed in MHD simulations and theoretical work) we can infer the black hole mass by constraining the transition region to occur at $10^{5}r_{s}$ in all jets (as in M87), shown in Figure \ref{corr3}. In this case we find black hole masses in the range $10^{7}-10^{10}M_{\odot}$ consistent with galaxy surveys. We also find that BL Lacs have smaller black hole masses than FSRQs and the linear relation between jet power and transition region radius means that all these blazars have approximately the same Eddington accretion fraction between $0.01-0.1L_{Edd}$. The scenario of a universal jet structure which scales linearly with black hole mass is appealing for its simplicity and is assumed in current state of the art GRMHD jet simulations (for example \cite{2009MNRAS.394.1182K}, \cite{2010ApJ...711...50T} and \cite{2012MNRAS.423.3083M}). There are two problems with this scenario however: the first is that this trend is not consistent with indirect measurements of black hole masses and the second is that this scenario doesn't explain the difference we find in bulk Lorentz factors between BL Lacs and FSRQs. Also, this does not tie in with the connection between accretion mode state and jet production from X-ray binaries or the expected correspondence of FRI and FRII jets to BL Lacs and FSRQs as we expect from unification. For these reasons we currently favour a bimodal accretion mode between BL Lacs and FSRQs linked to the FRI/FRII dichotomy. Obviously, the most direct way in which to settle this would be through a comparison to reliable black hole mass measurements for blazars. 

\section{Summary}

In this Chapter we have shown that our jet model with a magnetically dominated accelerating parabolic base transitioning to a slowly decelerating conical jet is able to fit to observations of blazar jets with unprecedented detail across all frequencies. This offers support for the emerging picture of jets motivated by observations and simulations. We find that in fitting to a large sample of blazar spectra we are able to constrain dynamic and structural properties of blazar jets. Our two main results are: the discovery of a linear correlation between the radius of the transition region of the jet and the jet power; a relation between the maximum bulk Lorentz factor and the distance over which the jet accelerates before reaching equipartition. These results allow us to understand the physical origin of the blazar sequence for the first time but also offer evidence for an accretion mode dichotomy in AGN analogous to that observed in X-ray binary systems and consistent with a correspondence between BL Lac and FSRQs, FRI and FRII jet properties and the mode of accretion.
\newpage
\section{Appendix A}

\begin{figure*}
	\centering
		\subfloat[J0137]{ \includegraphics[width=8cm, clip=true, trim=1.5cm 1cm 2.5cm 1.5cm]{J0137.pdf} }
		\subfloat[J0210]{ \includegraphics[width=8cm, clip=true, trim=1.5cm 1cm 2.5cm 1.5cm]{J0210.pdf} }	
\\
\subfloat[J0229]{ \includegraphics[width=8cm, clip=true, trim=1.5cm 1cm 2.5cm 1.5cm]{J0229.pdf} }
		\subfloat[J0238.4]{ \includegraphics[width=8cm, clip=true, trim=1.5cm 1cm 2.5cm 1.5cm]{J02384.pdf} }	
\\
\subfloat[J0238.6]{ \includegraphics[width=8cm, clip=true, trim=1.5cm 1cm 2.5cm 1.5cm]{J02386.pdf} }
\subfloat[J0349]{ \includegraphics[width=8cm, clip=true, trim=1.5cm 1cm 2.5cm 1.5cm]{J0349.pdf} }	
		
	\caption{The fits to the SEDs of the remaining 32 blazars with simultaneous multiwavelength observations and redshifts from \cite{2010ApJ...716...30A}, not fitted in Chapter 5. The model is able to fit very well to all of the spectra including radio observations.}
\label{fig51}
\end{figure*}

\begin{figure*}
	\centering
		
		\subfloat[J0423]{ \includegraphics[width=8cm, clip=true, trim=1.5cm 1cm 2.5cm 1.5cm]{J0423.pdf} }
		\subfloat[J0457]{ \includegraphics[width=8cm, clip=true, trim=1.5cm 1cm 2.5cm 1.5cm]{J0457.pdf} }
\\	
\subfloat[J0507]{ \includegraphics[width=8cm, clip=true, trim=1.5cm 1cm 2.5cm 1.5cm]{J0507.pdf} }
\subfloat[J0531]{ \includegraphics[width=8cm, clip=true, trim=1.5cm 1cm 2.5cm 1.5cm]{J0531.pdf} }	
\\
\subfloat[J0538]{ \includegraphics[width=8cm, clip=true, trim=1.5cm 1cm 2.5cm 1.5cm]{J0538.pdf} }
\subfloat[J0730]{ \includegraphics[width=8cm, clip=true, trim=1.5cm 1cm 2.5cm 1.5cm]{J0730.pdf} }	
\caption{}
		
\label{fig52}

\end{figure*}

\begin{figure*}
	\centering
		\subfloat[J0921]{ \includegraphics[width=8cm, clip=true, trim=1.5cm 1cm 2.5cm 1.5cm]{J0921.pdf} }
\subfloat[J1057]{ \includegraphics[width=8cm, clip=true, trim=1.5cm 1cm 2.5cm 1.5cm]{J1057.pdf} }	
\\
\subfloat[J1159]{ \includegraphics[width=8cm, clip=true, trim=1.5cm 1cm 2.5cm 1.5cm]{J1159.pdf} }
		\subfloat[J1221]{ \includegraphics[width=8cm, clip=true, trim=1.5cm 1cm 2.5cm 1.5cm]{J1221.pdf} }			
\\
\subfloat[J1229]{ \includegraphics[width=8cm, clip=true, trim=1.5cm 1cm 2.5cm 1.5cm]{J1229.pdf} }	
\subfloat[J1256]{ \includegraphics[width=8cm, clip=true, trim=1.5cm 1cm 2.5cm 1.5cm]{J1256.pdf} }
\caption{}	
		
\label{fig53}

\end{figure*}

\begin{figure*}
	\centering
\subfloat[J1310]{ \includegraphics[width=8cm, clip=true, trim=1.5cm 1cm 2.5cm 1.5cm]{J1310.pdf} }	
\subfloat[J1457]{ \includegraphics[width=8cm, clip=true, trim=1.5cm 1cm 2.5cm 1.5cm]{J1457.pdf} }		
\\
\subfloat[J1504]{ \includegraphics[width=8cm, clip=true, trim=1.5cm 1cm 2.5cm 1.5cm]{J1504.pdf} }	
		\subfloat[J1512]{ \includegraphics[width=8cm, clip=true, trim=1.5cm 1cm 2.5cm 1.5cm]{J1512.pdf} }		
\\
\subfloat[J1522]{ \includegraphics[width=8cm, clip=true, trim=1.5cm 1cm 2.5cm 1.5cm]{J1522.pdf} }	
\subfloat[Mkn501]{ \includegraphics[width=8cm, clip=true, trim=1.5cm 1cm 2.5cm 1.5cm]{Mkn501.pdf} }		
\caption{}
		

\label{fig54}

\end{figure*}

\begin{figure*}
	\centering
\subfloat[J1719]{ \includegraphics[width=8cm, clip=true, trim=1.5cm 1cm 2.5cm 1.5cm]{J1719.pdf} }
\subfloat[J1849]{ \includegraphics[width=8cm, clip=true, trim=1.5cm 1cm 2.5cm 1.5cm]{J1849.pdf} }				
\\
\subfloat[J2000]{ \includegraphics[width=8cm, clip=true, trim=1.5cm 1cm 2.5cm 1.5cm]{J2000.pdf} }
\subfloat[J2143]{ \includegraphics[width=8cm, clip=true, trim=1.5cm 1cm 2.5cm 1.5cm]{J2143.pdf} }		
\\
\subfloat[BLLac]{ \includegraphics[width=8cm, clip=true, trim=1.5cm 1cm 2.5cm 1.5cm]{BLLac.pdf} }	
\subfloat[J2254]{ \includegraphics[width=8cm, clip=true, trim=1.5cm 1cm 2.5cm 1.5cm]{J2254.pdf} }		
\caption{}		

\label{fig55}

\end{figure*}

\begin{figure*}
	\centering
		\subfloat[J2327]{ \includegraphics[width=8cm, clip=true, trim=1.5cm 1cm 2.5cm 1.5cm]{J2327.pdf} }	
		\subfloat[J2345]{ \includegraphics[width=8cm, clip=true, trim=1.5cm 1cm 2.5cm 1.5cm]{J2345.pdf} }	
\caption{}	
\label{fig56}

\end{figure*}
\newpage

\begin{sidewaystable}
\centering
\begin{tabular}{| c | c | c | c | c | c | c | c | c | c | c | c | c | c | c | c |}
\hline
Blazar & $W_{j}$(W) & $L$(m) & $ E_{\m{max}}$(MeV) & $\alpha$  & $\theta_{\m{observe}}$ & $\gamma_{\m{max}}$ & $\gamma_{\m{min}}$ & $ L_{\m{acc}}$(W) & $ R_{T}$(m) & $ B_{T}$(T)& $M(M_{\odot})$  \\ \hline 
J0035 & $5.0 \times 10^{37}$ & $10^{20}$ & $40.6$ & $1.3$ & $1^{0}$ & $14$ & $10$ & $1.67\times 10^{38}$ & $2.70\times 10^{14}$ & $5.91\times 10^{-5}$ & $7.69\times 10^{7}$ \\ \hline
J0137 & $7.06\times 10^{38}$ & $1\times 10^{21}$ & $22.8$ & $2.35$ & $1^{0}$ & $27$ & $16$ & $2.5\times 10^{38}$ & $1.21\times 10^{16}$ & $2.58\times 10^{-6}$ & $3.44\times 10^{9}$ \\ \hline
J0210 & $7.78\times 10^{38}$ & $2\times 10^{21}$ & $5.11$ & $2.01$ & $1^{0}$ & $38$ & $20$ & $4.27\times 10^{38}$ & $9.76\times 10^{15}$ & $2.38\times 10^{-6}$ & $2.78\times 10^{9}$ \\ \hline
J0222 & $1.04\times 10^{38}$ & $5\times 10^{20}$ & $16.2$ & $1.6$ & $1^{0}$ & $12$ & $8$ & $1.67\times 10^{38}$ & $1.47\times 10^{14}$ & $0.000184$ & $4.17\times 10^{7}$ \\ \hline
J0229 & $7\times 10^{38}$ & $1\times 10^{21}$ & $8.1$ & $1.9$ & $1^{0}$ & $40$ & $30$ & $4.17\times 10^{38}$ & $1.23\times 10^{16}$ & $1.7\times 10^{-6}$ & $3.5\times 10^{9}$ \\ \hline
J0238.4 & $1.2\times 10^{39}$ & $1\times 10^{21}$ & $8.1$ & $2.15$ & $1.2^{0}$ & $25$ & $15$ & $3.42\times 10^{38}$ & $3.27\times 10^{16}$ & $1.34\times 10^{-6}$ & $9.29\times 10^{9}$ \\ \hline
J0238.6 & $1.71\times 10^{39}$ & $1\times 10^{21}$ & $14.4$ & $2.01$ & $1^{0}$ & $38$ & $25$ & $5.7\times 10^{38}$ & $5.98\times 10^{15}$ & $5.78\times 10^{-6}$ & $1.69\times 10^{9}$ \\ \hline
J0349 & $1.67\times 10^{39}$ & $1\times 10^{21}$ & $6.74$ & $1.45$ & $1^{0}$ & $30$ & $8$ & $8.33\times 10^{38}$ & $1.48\times 10^{16}$ & $2.91\times 10^{-6}$ & $4.21\times 10^{9}$ \\ \hline
J0423 & $1\times 10^{39}$ & $2\times 10^{21}$ & $4.06$ & $2.11$ & $1^{0}$ & $30$ & $18$ & $1.99\times 10^{38}$ & $1.41\times 10^{16}$ & $2.37\times 10^{-6}$ & $4.01\times 10^{9}$ \\ \hline
J0457 & $8.5\times 10^{38}$ & $1\times 10^{21}$ & $8.1$ & $1.85$ & $1^{0}$ & $33$ & $20$ & $3.33\times 10^{38}$ & $3.52\times 10^{16}$ & $7.95\times 10^{-7}$ & $1\times 10^{10}$ \\ \hline
J0507 & $1.85\times 10^{37}$ & $2\times 10^{21}$ & $32.2$ & $1.5$ & $2^{0}$ & $16$ & $10$ & $8.55\times 10^{37}$ & $4.41\times 10^{13}$ & $0.000193$ & $1.26\times 10^{7}$ \\ \hline
J0531 & $2.17\times 10^{39}$ & $2\times 10^{21}$ & $2.87$ & $1.6$ & $1^{0}$ & $28$ & $13$ & $1.39\times 10^{39}$ & $4.40\times 10^{16}$ & $1.2\times 10^{-6}$ & $1.25\times 10^{10}$ \\ \hline
J0537 & $8.0\times 10^{37}$ & $1\times 10^{21}$ & $102$ & $1.75$ & $1.5^{0}$ & $12$ & $6$ & $1.25\times 10^{35}$ & $5.41\times 10^{14}$ & $4.36\times 10^{-5}$ & $1.54\times 10^{8}$  \\ \hline
J0538 & $1.78\times 10^{39}$ & $1\times 10^{21}$ & $10.2$ & $2.2$ & $1^{0}$ & $40$ & $22$ & $6.84\times 10^{38}$ & $2.20\times 10^{16}$ & $1.52\times 10^{-6}$ & $6.25\times 10^{9}$ \\ \hline
J0630 & $2.1\times 10^{38}$ & $1\times 10^{20}$ & $81$ & $1.3$ & $1$ & $14$ & $10$ & $1.25\times 10^{35}$ & $1.35\times 10^{15}$ & $2.42\times 10^{-5}$ & $3.85\times 10^{8}$ \\ \hline
J0730 & $2.14\times 10^{39}$ & $1\times 10^{21}$ & $4.55$ & $1.7$ & $1^{0}$ & $26$ & $15$ & $1.08\times 10^{39}$ & $3.06\times 10^{16}$ & $1.84\times 10^{-6}$ & $8.7\times 10^{9}$ \\ \hline
J0855 & $1.56\times 10^{38}$ & $5\times 10^{20}$ & $5.11$ & $1.63$ & $1^{0}$ & $8$ & $6$ & $8.33\times 10^{36}$ & $4.05\times 10^{14}$ & $0.000122$ & $1.15\times 10^{8}$ \\ \hline
J0921 & $1.91\times 10^{39}$ & $1\times 10^{21}$ & $8.1$ & $2.1$ & $1^{0}$ & $30$ & $18$ & $8.55\times 10^{38}$ & $1.30\times 10^{16}$ & $3.53\times 10^{-6}$ & $3.71\times 10^{9}$ \\ \hline
J1015 & $2.41\times 10^{37}$ & $1\times 10^{21}$ & $32.2$ & $1.5$ & $3.5^{0}$ & $10$ & $3$ & $2.5\times 10^{37}$ & $5.85\times 10^{13}$ & $0.000266$ & $1.66\times 10^{7}$ \\ \hline
J1057 & $9.41\times 10^{38}$ & $1\times 10^{21}$ & $4.06$ & $2.1$ & $1^{0}$ & $26$ & $20$ & $5.7\times 10^{37}$ & $1.11\times 10^{16}$ & $3.36\times 10^{-6}$ & $3.16\times 10^{9}$ \\ \hline
J1159 & $5.33\times 10^{38}$ & $2\times 10^{21}$ & $3.45$ & $1.95$ & $1^{0}$ & $30$ & $15$ & $1.14\times 10^{38}$ & $7.34\times 10^{15}$ & $3.31\times 10^{-6}$ & $2.09\times 10^{9}$ \\ \hline
J1221 & $1.71\times 10^{37}$ & $1\times 10^{21}$ & $32.2$ & $1.75$ & $2^{0}$ & $19$ & $10$ & $1.14\times 10^{37}$ & $2.22\times 10^{15}$ & $3.11\times 10^{-6}$ & $6.31\times 10^{8}$ \\ \hline
J1229 & $7.5\times 10^{39}$ & $1\times 10^{21}$ & $3.22$ & $1.2$ & $8.5^{0}$ & $12$ & $8$ & $1.97\times 10^{39}$ & $3.17\times 10^{15}$ & $7.22\times 10^{-5}$ & $9\times 10^{8}$ \\ \hline
J1256 & $1.64\times 10^{39}$ & $1\times 10^{21}$ & $3.22$ & $2.1$ & $1^{0}$ & $37$ & $18$ & $1.99\times 10^{38}$ & $1.76\times 10^{16}$ & $1.97\times 10^{-6}$ & $5.01\times 10^{9}$ \\ \hline

\end{tabular}
\caption{The values of the physical parameters used in the fits from this Chapter (shown in Figures $\ref{fig51}$--\ref{fig56}) and Chapter 5.}
\label{tab51}

\end{sidewaystable}

\begin{sidewaystable}
\centering
\begin{tabular}{| c | c | c | c | c | c | c | c | c | c | c | c | c | c | c | c |}
\hline

Blazar & $W_{j}$(W) & $L$(m) & $ E_{\m{max}}$(MeV) & $\alpha$  & $\theta_{\m{observe}}$ & $\gamma_{\m{max}}$ & $\gamma_{\m{min}}$ & $ L_{\m{acc}}$(W) & $ R_{T}$(m) & $ B_{T}$(T)& $M(M_{\odot})$  \\ \hline 
J1310 & $1.5\times 10^{39}$ & $1\times 10^{21}$ & $2.56$ & $1.95$ & $1^{0}$ & $50$ & $30$ & $2.28\times 10^{38}$ & $5.01\times 10^{15}$ & $4.89\times 10^{-6}$ & $1.43\times 10^{9}$ \\ \hline
J1312 & $2.3\times 10^{38}$ & $1\times 10^{21}$ & $81$ & $1.6$ & $1.2^{0}$ & $10$ & $6$ & $2.5\times 10^{34}$ & $1.62\times 10^{15}$ & $2.96\times 10^{-5}$ & $4.62\times 10^{8}$ \\ \hline
J1457 & $1.17\times 10^{39}$ & $1\times 10^{21}$ & $14.4$ & $2.05$ & $1^{0}$ & $36$ & $25$ & $5.7\times 10^{38}$ & $2.54\times 10^{16}$ & $1.18\times 10^{-6}$ & $7.22\times 10^{9}$ \\ \hline
J1504 & $2.04\times 10^{39}$ & $1\times 10^{21}$ & $17.3$ & $1.85$ & $1^{0}$ & $42$ & $16$ & $1.5\times 10^{39}$ & $5.92\times 10^{16}$ & $5.72\times 10^{-7}$ & $1.69\times 10^{10}$ \\ \hline
J1512 & $4.62\times 10^{38}$ & $2\times 10^{21}$ & $3.22$ & $1.9$ & $1^{0}$ & $45$ & $35$ & $7.69\times 10^{37}$ & $1.47\times 10^{16}$ & $1.03\times 10^{-6}$ & $4.18\times 10^{9}$ \\ \hline
J1522 & $6.52\times 10^{38}$ & $1\times 10^{21}$ & $5.73$ & $1.65$ & $1^{0}$ & $36$ & $18$ & $1.08\times 10^{38}$ & $3.12\times 10^{16}$ & $7.18\times 10^{-7}$ & $8.89\times 10^{9}$ \\ \hline
J1719 & $3.39\times 10^{37}$ & $1\times 10^{21}$ & $8.1$ & $2.2$ & $1^{0}$ & $45$ & $25$ & $1.42\times 10^{36}$ & $2.22\times 10^{15}$ & $1.85\times 10^{-6}$ & $6.31\times 10^{8}$ \\ \hline
J1751 & $2.08\times 10^{38}$ & $2\times 10^{21}$ & $4.06$ & $1.98$ & $1^{0}$ & $34$ & $18$ & $3.33\times 10^{37}$ & $6.45\times 10^{15}$ & $2.08\times 10^{-6}$ & $1.83\times 10^{9}$ \\ \hline
J1849 & $6.25\times 10^{38}$ & $1\times 10^{21}$ & $8.1$ & $2.2$ & $1^{0}$ & $40$ & $25$ & $8.55\times 10^{37}$ & $6.33\times 10^{15}$ & $3.13\times 10^{-6}$ & $1.79\times 10^{9}$ \\ \hline
J2000 & $2.8\times 10^{36}$ & $1\times 10^{21}$ & $128$ & $1.6$ & $4^{0}$ & $8$ & $4$ & $1.14\times 10^{37}$ & $3.52\times 10^{13}$ & $0.000188$ & $1\times 10^{7}$ \\ \hline
J2143 & $2.5\times 10^{37}$ & $5\times 10^{20}$ & $3.08$ & $1.45$ & $3^{0}$ & $10$ & $6$ & $1.14\times 10^{37}$ & $5.44\times 10^{13}$ & $0.000291$ & $1.55\times 10^{7}$ \\ \hline
J2158 & $1.55\times 10^{37}$ & $1\times 10^{20}$ & $51.1$ & $1.7$ & $2^{0}$ & $15$ & $7$ & $2.5\times 10^{37}$ & $1.01\times 10^{14}$ & $8.2\times 10^{-5}$ & $2.87\times 10^{7}$ \\ \hline
J2254 & $4.44\times 10^{39}$ & $3\times 10^{21}$ & $6.43$ & $2.05$ & $0.8^{0}$ & $60$ & $35$ & $2.28\times 10^{38}$ & $2.20\times 10^{16}$ & $1.6\times 10^{-6}$ & $6.25\times 10^{9}$ \\ \hline
J2327 & $1.23\times 10^{39}$ & $3\times 10^{21}$ & $1.81$ & $1.5$ & $0.8^{0}$ & $50$ & $32$ & $7.12\times 10^{38}$ & $3.98\times 10^{15}$ & $5.58\times 10^{-6}$ & $1.13\times 10^{9}$ \\ \hline
J2345 & $5\times 10^{38}$ & $2\times 10^{21}$ & $8.1$ & $1.95$ & $1.3^{0}$ & $50$ & $35$ & $5.7\times 10^{37}$ & $1.08\times 10^{16}$ & $1.3\times 10^{-6}$ & $3.06\times 10^{9}$ \\ \hline
Mkn421 & $6\times 10^{36}$ & $3\times 10^{20}$ & $338$ & $1.55$ & $3^{0}$ & $12$ & $9$ & $2.5\times 10^{36}$ & $2.22\times 10^{15}$ & $2.91\times 10^{-6}$ & $6.31\times 10^{8}$ \\ \hline
Mkn501 & $6.5\times 10^{36}$ & $1\times 10^{20}$ & $228$ & $1.68$ & $6.5^{0}$ & $9$ & $2$ & $8.55\times 10^{36}$ & $1.11\times 10^{14}$ & $8.06\times 10^{-5}$ & $3.16\times 10^{7}$ \\ \hline
BL Lac & $9\times 10^{36}$ & $5\times 10^{20}$ & $8.1$ & $1.95$ & $3^{0}$ & $8$ & $5$ & $8.33\times 10^{36}$ & $4.43\times 10^{13}$ & $0.000268$ & $1.26\times 10^{7}$ \\ \hline

\end{tabular}

\end{sidewaystable}
